Specification and Inference of Trace Refinement Relations

Modern software is constantly changing. Researchers and practitioners are increasingly aware that verification tools can be impactful if they embrace change through analyses that are compositional and span program versions. Reasoning about similarities and differences between programs goes back to Benton, who introduced state-based refinement relations, which were extended by Yang and others. However, to our knowledge, refinement relations have not been explored for traces. We present a novel theory that allows one to perform compositional reasoning about the similarities/differences between how fragments of two different programs behave over time through the use of what we call trace-refinement relations. We take a reactive view of programs and found Kleene Algebra with Tests (KAT) [Kozen] to be a natural choice to describe traces since it permits algebraic reasoning and has built-in composition. Our theory involves a two-step semantic abstraction from programs to KAT, and then our trace refinement relations correlate behaviors by (i) categorizing program behaviors into trace classes through KAT intersection and (ii) correlating atomic events/conditions across programs with KAT hypotheses. We next describe a synthesis algorithm that iteratively constructs trace-refinement relations between two programs by exploring sub-partitions of their traces, iteratively abstracting them as KAT expressions, discovering relationships through a custom edit-distance algorithm, and applying strategies (i) and (ii) above. We have implemented this algorithm as {\sc knotical}, the first tool capable of synthesizing trace-refinement relations. It built from the ground up in Ocaml, using InterProc and SymKAT. We have demonstrated that useful relations can be efficiently generated across a suite of 37 benchmarks that include changing fragments of array programs, systems code, and web servers.

==> Makefile <==
# A standard Makefile for latex stuff; this can be used as a template. 

ALL = paper.pdf
GRAPHS = 
PAPERTYPE = letter
LATEX = pdflatex
#LATEX = latex

all: $(ALL)

.SUFFIXES: .pic .tex .ps .dvi .bib .bbl

# %.ps: %.dvi $(GRAPHS)
# 	@# Using "-Ppdf" is supposed to make the PDF come out better,
# 	@# but it seems to screw up a few symbols in the PS file.
# 	@# FIX: Use -G0 as an argument to dvips!  See below.
# 	dvips -t $(PAPERTYPE) $< -o $@

# %.pdf: %.ps
# 	ps2pdf14 -dPDFSETTINGS=/prepress -dEmbedAllFonts=true $<

# %.pdf: %.dvi
# 	dvipdfmx $<

#%.bbl: %.bib
#        @@echo Building bibliography...
#        BIBINPUTS=$(BIBINPUTS):./bibs bibtex $(<:.bib=)

%.bbl: %.bib
	bibtex $(<:.bib=)

#paper.dvi: paper.tex 
paper.pdf: paper.tex *.tex 
	$(LATEX) $<
	@if [ "`grep 'undefined' $(<:.tex=.log) | grep -v 'Font Warning'`" != "" ] ; \
	then \
	  echo bibtex $(<:.tex=);\
	  bibtex -min-crossrefs=99 $(<:.tex=);\
	  echo $(LATEX) $<;\
	  $(LATEX) $<;\
	fi
	@if [ "`grep 'undefined' $(<:.tex=.log)` | grep -v 'Font Warning'" != "" ] ; \
	then \
	  echo bibtex $(<:.tex=);\
	  bibtex -min-crossrefs=99 $(<:.tex=);\
	  echo $(LATEX) $<;\
	  $(LATEX) $<;\
	fi
	@if [ "`grep 'undefined' $(<:.tex=.log)` | grep -v 'Font Warning'" != "" ] ; \
	then \
	  echo $(LATEX) $<;\
	  $(LATEX) $<;\
	fi
	@# Anything undefined past here is really undefined
	@if [ "`grep 'may have changed' $(<:.tex=.log)`" != "" ] ; \
	then \
	  echo $(LATEX) $<;\
	  $(LATEX) $<;\
	fi
	@if [ "`grep 'may have changed' $(<:.tex=.log)`" != "" ] ; \
	then \
	  echo $(LATEX) $<;\
	  $(LATEX) $<;\
	fi
	@if [ "`grep 'may have changed' $(<:.tex=.log)`" != "" ] ; \
	then \
	  echo $(LATEX) $<;\
	  $(LATEX) $<;\
	fi

clean:
	-rm -f *.aux *.dvi *.log *.bbl *.blg

veryclean: clean
	-rm -f *.ps *.pdf




all:
	pdflatex paper.tex && bibtex paper && pdflatex paper.tex && pdflatex paper.tex



==> definitions-kat.tex <==
%!TEX root = paper.tex
\section{Definitions}

{\bf General}

Given sets $S_1,\ldots,S_n$, a set $S\subseteq S_1\times S_2\times\ldots S_n$, and an element $s=(s_1,\ldots,s_n)\in S$ we denote with $\proj{i}{s}$ the projection of $s$ to its $i$-th element $s_i$ in $S_i$. We abuse notation and more generally we denote with $\proj{i}{S}$, the set $\{s_i\in S_i\mid s_i\in\proj{i}{s}, s\in S\}$.

Let $S$ be a set, $A$ and $B$ be subsets of $S$, and let $T_1\subseteq S\times S$ and $T_2\subseteq S\times S$ be two binary left-total relations over $S$. We denote with $T_1\circ_{A,B} T_2$, the \emph{composition} of $T_1$ and $T_2$ induced by $A$ and $B$ and is defined as the set $\{(p,r)\in S\times S\mid (p,r)\in T_1\textrm{ or }(p,r)\in T_2\textrm{ or }p\in A\textrm{ and }r\in B\}$.

\subsection{Programs}

We assume a set $\progs$ of (essentially imperative) \emph{programs} operating on a set $\states$ of \emph{states}.  We assume a distinguished ``error state'' $\fault \in \states$. A \emph{configuration} is a pair $\config{C}{\sigma}$, where $C$ is a program and $\sigma$ a state; we write $\configs$ for the set of all configurations. We assume a binary relation $\mathord{\leadsto} \subseteq \configs \times \states$ capturing the ``big step'', nondeterministic operational semantics of our programs; the statement $\config{C}{\sigma} \leadsto \rho$ should be read as meaning that executing program $C$ in initial state $\sigma$ can result in the final state $\rho$.  We say that the configuration $\config{C}{\sigma}$ \emph{goes wrong} if $\config{C}{\sigma} \leadsto \fault$, and is \emph{safe} otherwise.

\timos{Define boolean programs and say we assume this is the type of programs we consider in what follows.}

\subsection{Abstract Transition Systems}

\timos{Basic definitions about abstract transition systems.}

An \emph{abstract transition system} over a finite set of atomic propositions $\ap$ is a tuple $\ats = (\states, \initstates, \transitions, \labels)$, where $\states$ is a finite set of states, $\initstates\subseteq\states$ is the set of initial states, $\transitions$ is a total relation over $\states\times\states$ and $\labels$ is a mapping from $\states$ to $\powset{\ap}$. A \emph{path} $\path$ of the transition system $\ap$ is a sequence of states $s_0,s_1,\ldots,s_n,\ldots$, such that for all $i\in\mathbb{N}$, $s_0\in\initstates$ and $(s_i,s_{i+1})\in\transitions$. A \emph{word} derived from a path $\path=s_0,s_1,\ldots$ is the sequence $\labels(s_0),\labels(s_1),\labels(s_2),\ldots\in (\powset{\ap})^{\omega}$. For a path $\path$ we denote with $\labels(\path)$ its derived word. The language of an abstract transition system $\ats$ is the set $\{w\in(\powset{\ap})^{\omega}\mid w=\labels(\path), \textrm{ where }\path\textrm{ is a path of }\ats \}$. We denote the language of $\ats$ by $\lang{\ats}$.

Let $A\subseteq \ap$. Then, for any $\labels:\states\rightarrow\powset{\ap}$, we denote with $\labels_{|A}$ the function that maps any $s\in\states$ to $\labels(s)\cap A$. The \emph{projection} of a language $\lang{\ats}$, for $\ats=(\states,\initstates,\transitions,\labels)$, to a subset $A$ of $\ap$ is the language $\lang{\ats_{|A}}$, where $\ats_{|A}=(\states,\initstates,\transitions,\labels_{|A})$.

For $\ats$ an abstract transition system, we may declare a subset $\finalstates$ of the set $\states$, to be the set of \emph{final states}. We denote such an $\ats$ as the tuple $(\states, \initstates, \finalstates, \transitions, \labels)$. For two abstract transition systems $\ats_{1}=(\states_1,\initstates_1,\finalstates_1,\transitions_1,\labels_1)$ and $\ats_{2}=(\states_2,\initstates_2,\finalstates_2,\transitions_2,\labels_2)$, with $S_1$ and $S_2$ disjoint, we define their \emph{composition} to be $\ats=(\states_1\cup \states_2,\initstates_1,\finalstates_2,\transitions_1\circ_{\finalstates_1,\initstates_2}\transitions_2,\labels_1\cup\labels_2)$.

\subsection{Kleene Algebra with Tests}

A \emph{Kleene Algebra with Tests} $\kat$ is a two-sorted structure $(\Sigma,\bkat,+,\cdot,\kstar{},\kneg{},0,1)$, where $(\Sigma,+,\cdot,\kstar{},0,1)$ is a Kleene algebra, $(\bkat,+,\cdot,\kneg{},0,1)$ is a boolean algebra, and $(\bkat,+,\cdot,0,1)$ is a sub-algebra of $(\Sigma,+,\cdot,0,1)$.

We distinguish between two sets of symbols. A set $\actions$ for primitive actions, and a set $\tests$ for primitive tests. We define the grammar $\boolgr$ of Boolean test expressions as:

$$\boolgr\grdef b\in\tests\mid b_1\cdot b_2\mid b_1+b_2\mid \kneg{b}\mid 0\mid 1$$

and we define the grammar $\katgr$ of KAT expressions as:

$$\katgr\grdef p\in\actions\mid b\in\boolgr\mid k_1\cdot k_2\mid k_1+k_2\mid \kstar{k}\mid 0\mid 1$$

The Kleene algebra with tests over $\actions\cup\tests$, is obtained by quotienting $\boolgr$ with the axioms of Boolean algebras, and $\katgr$ with the axioms of Kleene Algebra. For $e,f\in \katgr$, we write $e\leq f$ if $e+f\equiv f$.

\timos{Define here how to obtain a KAT expression $k$ given a program $C$.}

\timos{We could get the following from literature:}

\begin{proposition}
	Given a program $C$ and a KAT expression $k$ over $\kat$ that corresponds to $C$, then for any precondition $P$ and postcondition $Q$, with respective boolean tests $b_P$ and $b_Q$ in $\bkat$, it holds that $\prepostprogram{P}{Q}{C}$ if and only if $b_P\cdot k\leq k\cdot b_Q$.
\end{proposition}


\begin{definition}[Intersection]
	Given a KAT $\kat$ and two of its elements $k_1$ and $k_2$ we define $k_1\cap k_2$ to be equal to $l_1+\ldots +l_n$, where $\{l_i\}_{i\leq n}$ is the set of all elements $l_i$ in $\kat$ such that $l_i\leq k_1$ and $l_i\leq k_2$.
\end{definition}

% \begin{example}
% 	Let $k$ be an element of the KAT $\kat$, and let $b_1,b_2$ be elements in $\bkat$. Then $k\cap (b_1\cdot k + b_2\cdot k)=b_1\cdot k + b_2\cdot k$.
% \end{example}

\subsection{Program Refinement}

\timos{Original definition. Adapt to our setting.}


\begin{definition}\label{def:refinement}
Let $C_1$ and $C_2$ be programs.  We say that $C_1$ \emph{refines} $C_2$, written $\refines{C_1}{C_2}$, if the following two conditions are met, for any state $\sigma$:
\begin{enumerate}
\item if $\config{C_1}{\sigma}$ goes wrong, then so does $\config{C_2}{\sigma}$;
\item if $\config{C_1}{\sigma} \leadsto \rho$, then either $\config{C_2}{\sigma} \leadsto \rho$, or $\config{C_2}{\sigma}$ goes wrong.
\end{enumerate}
\end{definition}

\timos{I believe the definition above is equivalent to:}

\begin{definition}\label{def:refinement-changed}
Let $C_1$ and $C_2$ be programs.  We say that $C_1$ \emph{refines} $C_2$, written $\refines{C_1}{C_2}$, if for any $\sigma\in\states$ and $\rho\in\states\cup\{\fault\}$. If $\config{C_1}{\sigma} \leadsto \rho$, then either $\config{C_2}{\sigma} \leadsto \rho$, or $\config{C_2}{\sigma}\leadsto \fault$.
\end{definition}

We define an \emph{interface} to be an equivalence relation on the set of states $\states$.

\begin{definition}
\label{def:absrefines}
Let $I$ and $O$ be interfaces, and $C,C'$ be programs.  We say that \emph{$C'$ refines $C$ w.r.t.\ $(I,O)$}, written $\absrefines{C'}{C}{I}{O}$, if the following two conditions are met, for all states $\sigma,\sigma'$ such that $I(\sigma,\sigma')$:
\begin{enumerate}
\item if $\config{C'}{\sigma'}$ goes wrong, then so does $\config{C}{\sigma}$;
\item if $\config{C'}{\sigma'} \leadsto \rho'$, then either there exists $\rho$ such that $\config{C}{\sigma} \leadsto \rho$ and $O(\rho,\rho')$, or else $\config{C}{\sigma}$ goes wrong.
\end{enumerate}
\end{definition}

\timos{Talk about Benton here. Possibly mention results from stapler work too, but mention they are unpublished.}



==> implementation.tex <==
%!TEX root = paper.tex
\section{Implementation}\label{sec:implementation}

\todo{All this in the evaluation section.}
We have realized our algorithm in a prototype tool called {\knotical}.
Our tool is written in {\ocaml}, using {\interproc} as an
abstract interpreter, and {\symkat} as a symbolic solver for
KAT equalities~\cite{symkat,symkattool}.
%\timos{Describe {\interproc} and {\symkat} briefly.} % EJK says: probably not needed
We now describe implementation choices made for the subcomponents  described in Section~\ref{subsec:subprocedures}.

\paragraph{Solution Trees.}
\todo{Solution trees in the evaluation section.}
Our tool {\knotical} generates multiple solutions, internally represented in the form of a tree. During the {\akatdiff} and {\asolvediff} steps of the algorithm, multiple choices can be made and each solution tree corresponds to a particular set of choices. The solution shown in Figure~\ref{fig:solution} is just one of the 75 solutions generated.
%
Branching in a solution tree corresponds to the different restrictions applied to the programs and their complement. For example, one branch could correspond to a decision to explore the behaviors when we assume a particular variable to be $\true$, whereas the other branch would correspond to the behaviors that result from assuming that variable is $\false$.
%
Often the solution trees (or subtrees) are partial, in the sense that the different restrictions applied to the programs, when taken together do not cover all behaviors of the input program. As explained in Remark~\ref{rem:trivial-solution}, these partial solutions can readily be converted to complete ones.

\Tremoved{\paragraph{Implementation of algorithm subcomponents.}
We now describe the implementations of the subcomponents, as well as their limitations, in more detail. As noted, the overall algorithm is parameterized by whether we are looking for solutions to equivalence ($\equiv_{\hypotheses}$), or simply to inclusion ($\leq_{\hypotheses}$). The functionality of the sub-procedures described below is largely the same for the two cases, and we give details only when it differs.}

\vskip5pt
\noindent
\Tremoved{
{\bf ${\atranslate}(C,\alpha)$:} This procedure is given a (possibly restricted) program $C$ and an abstraction $\alpha=(\kat,A_S,\alpha_S,\alpha_B)$ as input. We run {\interproc} to populate the locations of the program with invariants that hold at those locations according to the abstraction $\alpha$. This information in turn is used in converting the abstract program into a KAT expression $k$ in $\kat$ that covers its behavior. Semantic information is mostly exploited in the cases where paths of the program are determined to be infeasible. For example, consider the simple \emph{instrumented} program}
\begin{displaymath}
\begin{array}{l}
	\texttt{assume(d==0); c=d;}\\
	\texttt{if (c==0) \{ execB(); \} else \{ execD();\}}
\end{array}
\end{displaymath}
\Tremoved{% $$\texttt{assume(d==0); c=d; if (c==0) \{ execB(); \} else \{ execD();\}}.$$
The standard syntactic translation~\cite{kozen} alone, would produce the expression $\kM{c}{d==0}\cdot\kM{E}{c=d}\cdot(\kM{c}{c==0}\cdot\kM{B}{execB}+\overline{\kM{c}{c==0}}\cdot\kM{D}{execD}).$ In our case, {\interproc} will determine that the condition $\textsf{c==0}$ is always true under the instrumented assumption $\texttt{assume(d==0)}$ and the program in such a case is converted to the much simpler expression $\kM{B}{execB}$ instead.}

\vskip5pt
\noindent
\Tremoved{
{\bf ${\akatdiff}(k_1$,$k_2$,$\hypotheses)$:}
For this sub-procedure we use the {\symkat} library~\cite{symkattool}. Given two KAT expressions $k_1$ and $k_2$ as input, as well as a set of hypotheses, we feed them into the library to get a \emph{singleton} set {\acexs} comprising either a single string $c$ in $\katminus{k_1}{k_2}{\hypotheses}$ when we ask for inclusion of one input program to the other, or a pair of strings $(c_1,c_2)$, with $c_1$ in $\katminus{k_1}{k_2}{\hypotheses}$ and $c_2$ in $\katminus{k_2}{k_1}{\hypotheses}$, when we ask for equivalence of the two input programs. As an example, if $k_1=a\cdot M\cdot (b\cdot F+\overline{b}\cdot G)$ and $k_2=a\cdot M\cdot\overline{b}\cdot G$, then the string $a\cdot M\cdot b\cdot F$ is included in $k_1$ but not in $k_2$, and thus in $\katminus{k_1}{k_2}{\hypotheses}$.}
%Such a string then may be returned by {\symkat}, when given the two KAT expressions as input, and a set of hypotheses (in this case an empty set).

\vskip5pt
\noindent
\Tremoved{
{\bf ${\asolvediff}(k_1,k_2,\hypotheses,{\acexs})$:} {\acexs} is either a pair of strings $(c_1,c_2)$ such that $c_1$ is in $\katminus{k_1}{k_2}{\hypotheses}$ and $c_1\in\katminus{k_2}{k_1}{\hypotheses}$, (when searching for equivalence) or a single string $c\in\katminus{k_1}{k_2}{\hypotheses}$ (when searching for refinement/inclusion). We apply a  customized edit-distance algorithm discussed (Section~\ref{sec:edit-distance}), which returns a set of \emph{transformations} that can be applied to two KAT strings $c_1$ and $c_2$ to make them equivalent. These transformations are in the form of removing alphabet symbols from the strings at particular locations, or replacing some symbol with another. From these transformations, {\asolvediff} constructs a list of restrictions to be applied on the input programs of the form $(r_1,r_2,\hypotheses)$, where $r_1$ and $r_2$ are KAT expressions, and $\hypotheses$ is a set of hypotheses.}

\Tremoved{When the edit-distance algorithm asks for the removal of an alphabet symbol from, say, string $c_1$, we consider two cases, depending on whether the symbol corresponds to a boolean condition or not. If so, the KAT expression $r_1$ corresponding to this transformation is essentially obtained by adding a hypothesis inserting the valuation of the boolean variable, in the given KAT expression $k_1$. Since in some cases we want these restrictions to cover all behaviors of the input programs, we also consider the negation of that valuation. As such, at least two restrictions are considered in this way, namely $(r_1,r_2,\hypotheses)$ and $(r_1',r_2,',\hypotheses')$, such that $r_1$ and $r_1'$ cover $k_1$. On the other hand, when the removal of an event $\kM{M}{}$ is required, a hypothesis of the form $\kM{M}{}\equiv 1$ is added to the set of hypotheses $\hypotheses$. The types of hypotheses we consider in this step, are also somewhat limited by the use of {\symkat}, as well as because of more general undecidability concerns.
As such, hypotheses such as $\kM{M}{}\kM{N}{}\equiv \kM{N}{}\kM{M}{}$, expressing that the two events $\kM{M}{}$ and $\kM{N}{}$ commute, are not allowed.}

\vskip5pt
\noindent
\Tremoved{
{\bf $\arestrict(C_1,r_1,C_2,r_2,\hypotheses,\alpha)$:} We use each restriction tuple $(r_1,r_2,\hypotheses)$ in the set returned by $\asolvediff$ to apply the restriction on the input programs $C_1$ and $C_2$. The sub-procedure, thus, takes as input the two programs $C_i$, as well as the respective KAT expression $r_i$, and produces a new program $D_i$ whose behaviors are restricted accordingly, as well as a new common abstraction $\alpha'$ that refines $\alpha$. In our implementation, we restrict programs with a form of cross-product construction, in which \texttt{assume} statements are instrumented on appropriate lines of code. 
For example, for a program of the form}
$$k=(\kkttb\cdott\kkttO+\overline{\kkttb}\cdott1)^*,$$
\Tremoved{we can implement the restriction}
$$l=(\kkttb\cdot (\kkttb\cdott\kkttO+\overline{\kkttb}\cdott1))^*=(\kkttb\cdott\kkttO)^*$$
\Tremoved{with an \texttt{assume(l==true)} instrumented immediately inside the body of the corresponding while loop.}



==> refinement-kat.tex <==
%!TEX root = paper.tex
\section{KAT Representations and Refinements}
\label{sec:refinement}

One of the main goals behind KAT representation of programs is checking that two formulas are equivalent using equational proofs. Thus, given $k_1$ and $k_2$, and using the axioms of the underlying Kleene Algebra with Tests, one may be able to show that $k_1\equiv k_2$. In this work, we use this equational approach to express that two programs given in the form of two KAT formulas, have the same behavior.


\begin{definition}\label{def:concretekrefine}
	Let $k_1$ and $k_2$ be two KAT formulas over $\kat$. We say that $k_1$ \emph{refines} $k_2$, and denote it by $\refines{k_1}{k_2}$, if for any $b,d\in\bkat$:
	\begin{enumerate}
		\item $b\cdot k_1\equiv 0$ implies $b\cdot k_2\equiv 0$,
		\item $b\cdot k_1\cdot d\not\equiv 0$ implies $b\cdot k_2\cdot d\not\equiv 0$, or $b\cdot k_2\equiv 0$.
	\end{enumerate}
\end{definition}

For programs over actions $A$ and with state space $\states$, we associate a KAT $\kat$, in such a way that there is an injective mapping $\statetobool{}$ from the set of states $\states$ to the boolean subalgebra $\bkat$ of $\kat$, such that:
\begin{enumerate}
	\item for any program over this state space and set of actions, and for any $\sigma,\rho\in\states$, $\config{C}{\sigma}\leadsto{\rho}$ if and only if $\statetobool{\sigma}\cdot k_C\cdot \statetobool{\rho}\not\equiv 0$
	\item for any $b\in\bkat$ and state $\sigma$, with $b\neq\statetobool{\sigma}$, if $b\leq\statetobool{\sigma}$ then $b\equiv 0$
	\item for any $b\in\bkat$ different from $0$ there exists a state $\sigma$, with $\statetobool{\sigma}\leq b$.\timos{Is this condition too much?}
\end{enumerate}

\timos{Maybe the last two conditions above can be summarized as: for any $b\in\bkat$ different from $0$, there exist states $\sigma_1,\ldots\sigma_n$ such that $b=(\statetobool{\sigma_1}+\ldots+\statetobool{\sigma_n})$.}

\timos{Write the above as a definition}

\begin{definition}\label{def:program-to-kat}
	Translation of a program $C$ over $\states$ to an element $k$ of a KAT $\kat$.
\end{definition}

\begin{theorem}
	Let $C_1$ and $C_2$ be two programs over states $\states$, and let $k_1$ and $k_2$ be the two KAT formulas that correspond to the two programs respectively. Then it holds that $\refines{C_1}{C_2}$ if and only if $\refines{k_1}{k_2}$.
\end{theorem}

\begin{proof}
	For the {\it only if} direction, suppose that $\refines{C_1}{C_2}$ and pick any $b,d\in\bkat$. Suppose first that $b\cdot k_1\equiv 0$. Then let $\sigma_1,\ldots,\sigma_n$ be the set of states such that $\statetobool{\sigma_1}+\ldots+\statetobool{\sigma_n}\equiv b$ for $i\leq n$. Then, for all $i\leq n$, $\config{C_1}{\sigma_i}$ goes wrong which implies that $\config{C_2}{\sigma_i}$ also goes wrong by assumption that $\refines{C_1}{C_2}$. This means that for all $i\leq n$, $\statetobool{\sigma_i}\cdot k_2\equiv 0$, and thus $b\cdot k_2\equiv\statetobool{\sigma_1}+\ldots+\statetobool{\sigma_n}\cdot k_2\equiv 0$.
	
	The second condition states that $b\cdot k_1\cdot d\not\equiv 0$ implies $b\cdot k_2\cdot d\not\equiv 0$, or $b\cdot k_2\equiv 0$.
	Assume that $b\cdot k_1\cdot d\not\equiv 0$. Let $\sigma_1,\ldots,\sigma_n$ be the set of states such that $b=\statetobool{\sigma_1}+\ldots+\statetobool{\sigma_n}$, and let $\rho_1,\ldots,\rho_m$ be the set of states such that $d=\statetobool{\rho_1}+\ldots+\statetobool{\rho_m}$. Therefore, $(\statetobool{\sigma_1}+\ldots+\statetobool{\sigma_n})\cdot k_1\cdot (\statetobool{\rho_1}+\statetobool{\rho_m})\not\equiv 0$. Let $(\sigma_i,\rho_j)$ be all the pairs, such that $\statetobool{\sigma_i}\cdot k_1\cdot\statetobool{\rho_j}\not\equiv 0$. It follows by definition that $\config{C_1}{\sigma_i}\leadsto\rho_j$. Therefore, either $\config{C_2}{\sigma_i}\leadsto\rho_j$ or $\config{C_2}{\sigma_i}\leadsto\fault$ by assumption that $\refines{C_1}{C_2}$. It follows that $b\cdot k_2\equiv(\statetobool{\sigma_1}+\ldots+\statetobool{\sigma_n})\cdot k_2\equiv 0$ or $b\cdot k_2\cdot d\equiv(\statetobool{\sigma_1}+\ldots+\statetobool{\sigma_n})\cdot k_2\cdot (\statetobool{\rho_1}+\ldots+\statetobool{\rho_m})\not\equiv 0$, as required.
	
	% By Lemma~\ref{}, it follows that $\config{C_1}{\bstate{b}}\leadsto\bstate{d}$. By assumption that $\refines{C_1}{C_2}$, it holds that $\config{C_2}{\bstate{b}}\leadsto\bstate{d}$ or $\config{C_1}{\bstate{b}}$ goes wrong. Again by Lemma~\ref{}, it follows that $b\cdot k_2\leq k_2\cdot d$ or $b\cdot k_2 = 0$, as required.
	
	% Now let $b$ and $d$ be any elements in $\bkat$. We write $b=b_1+\ldots +b_n$ and $d=d_1+\ldots +d_n$ such that $b_i,d_j\in\basebkat$, for $i\in[n]$ and $j\in[m]$. Suppose $b\cdot k_1\leq k_1\cdot d$. Then, $(b_1+\ldots+b_n)\cdot k_1\leq k_1\cdot (d_1+\ldots+d_m)$.
	
	For the {\it if} direction, suppose that $\refines{k_1}{k_2}$, and let $\sigma,\rho$ be any two states in $\states$. If $\config{C_1}{\sigma}\leadsto\fault$, then $\statetobool{\sigma}\cdot k_1\equiv 0$. By the assumption that $\refines{k_1}{k_2}$, we have that $\statetobool{\sigma}\cdot k_2\equiv 0$. Therefore, $\config{C_2}{\sigma}\leadsto\fault$. On the other hand, if $\config{C_1}{\sigma}\leadsto\rho$, then $\statetobool{\sigma}\cdot k_1\cdot\statetobool{\rho}\not\equiv 0$. By the assumption that $\refines{k_1}{k_2}$, it follows that $\statetobool{\sigma}\cdot k_2\cdot\statetobool{\rho}\not\equiv 0$ or $\statetobool{\sigma}\cdot k_2\equiv 0$. Therefore, $\config{C_2}{\sigma}\leadsto\rho$ or $\config{C_2}{\sigma}\leadsto\fault$, as required.
\end{proof}

A KAT interface is a tuple $(I,\hypotheses,O)$, where $I$ and $O$ are boolean subalgebras of $\bkat$, and $\hypotheses$ is a set of hypotheses.

\begin{definition}
	Let $k_1$ and $k_2$ be two KAT formulas over $\kat$. We say that $k_1$ \emph{state-refines} $k_2$ with respect to $(I,\hypotheses,O)$, and denote it by $\absstatekrefines{k_1}{k_2}{I}{O}{\hypotheses}$, if for any $b\in I$ and $d\in O$:
	\begin{enumerate}
		\item $b\cdot k_1\equiv_{\hypotheses} 0$ implies $b\cdot k_2\equiv_{\hypotheses} 0$,
		\item $b\cdot k_1\leq_{\hypotheses} k_1\cdot d$ implies $b\cdot k_2\leq_{\hypotheses} k_2\cdot d$, or $b\cdot k_2\equiv_{\hypotheses} 0$.
	\end{enumerate}
\end{definition}

When $\hypotheses=\emptyset$, we simply write $\absstatekrefines{k_1}{k_2}{I}{O}{}$. Notice that for $I$ and $O$ being the Boolean Algebra $\bkat$, and any two KAT formulas $k_1,k_2$ over $\kat$, it holds that $\refines{k_1}{k_2}$ if and only if $\absstatekrefines{k_1}{k_2}{I}{O}{}$.

% \begin{definition}
% 	Let $k_1$ and $k_2$ be two KAT formulas over $\kat$. We say that $k_1$ \emph{trace-refines} $k_2$, or simply $k_1$ \emph{refines} $k_2$, with respect to $(I,\hypotheses,O)$, and denote it by $\abskrefines{k_1}{k_2}{I}{O}{\hypotheses,k}$, if for any $b\in I$ and $d\in O$, $$b\cdot k_1\cdot d\leq_{\hypotheses} b\cdot k_2\cdot d.$$
% \end{definition}

\timos{Below is the old definition of refinement.}

Let $\kat$ be a Kleene Algebra, and let $K$ be a subset of its elements. We say that $K=\{k_1,\ldots,k_n\}$ is a \emph{partition} of $\kat$, if $k_1+\ldots +k_n=1$, and for any two distinct elements $k_i,k_j\in K$, and any $k\in\kat$, if $k\leq k_i$ and $k\leq k_j$, then $k=0$. We use the same terminology for Boolean algebras.

\begin{definition}\label{def:kat-refinement}
	Let $\bkat'_1,\bkat'_2$ be partitions of the boolean algebra $\bkat$, let $\hypothesesclass$ be a set of hypotheses over $\kat$, and let $\interfaceRel$ be a total mapping from $\bkat'_1$ to $\bkat'_2\times\powset{\hypothesesclass}$.
	Given two KAT formulas $k_1$ and $k_2$ over $\kat$, we say that $k_1$ \emph{trace-refines} $k_2$, or simply $k_1$ \emph{refines} $k_2$, with respect to $I$, and denote it by $\abskrefines{k_1}{k_2}{\interfaceRel}{}{}$, if for any $b_1\in \bkat'_1$, $$b_1\cdot k_1\leq_{\hypotheses} b_2\cdot k_2,$$
	where $(b_2,\hypotheses)=\interfaceRel(b_1)$.
\end{definition}

For readability, we split the total mapping $\interfaceRel$ into two components $\interfaceBool$ and $\interfaceHypotheses$, such that for any $b\in\domain{\interfaceRel}$, $\interfaceRel(b)=(\interfaceBool(b),\interfaceHypotheses(b))$.

\timos{new definition below}

Let $k$ be an element of a KAT $\kat$. We say a set $S=\{s_1,\ldots,s_n\}$ of $\kat$ elements \emph{partitions} $k$, if $k=s_1+\ldots s_n$, and for any distinct $s_i,s_j\in S$, and any element $s\in\kat$, if $s\leq s_i$ and $s\leq s_j$ then $s=0$.

\begin{definition}\label{def:kat-refinement}
	Let $\kat$ be a KAT, let $\hypotheses$ be a set of hypotheses over $\kat$, and let $\interfaceRel$ be a relation over $\kat\times\kat\times\powset{\hypotheses}$.
	Given two KAT elements $k_1$ and $k_2$ of $\kat$, we say that $k_1$ \emph{trace-refines} $k_2$, or simply $k_1$ \emph{refines} $k_2$, with respect to $\interfaceRel$, and denote it by $\abskrefines{k_1}{k_2}{\interfaceRel}{}{}$, if for any $(l_1,l_2,A)\in \interfaceRel$, $$l_1\cap k_1\leq_{A} l_2\cap k_2,$$ and $\proj{1}{\interfaceRel}$ partitions $k_1$.
\end{definition}


\subsection{Composition}
\label{subsec:composition}

Let $k_1,k_2\in\kat$ and $I$ be such that $\abskrefines{k_1}{k_2}{\interfaceRel}{}{}$. We denote with $\interfacePost$ the function that maps each $b_1\in\domain{\interfaceRel}$ to a pair $(d_1,d_2)\in\bkat\times\bkat$, such that $b_2=\interfaceBool(b_1)$ and $A=\interfaceHypotheses(b_1)$, and where $b_1\cdot k_1\leq_{A} k_1\cdot d_1$ and $b_2\cdot k_2\leq_{A} k_2\cdot d_2$, and there is no $d'$ such that $b_1\cdot k_1\leq_{A} k_1\cdot d'$ and $d'< d_2$ or $b_2\cdot k_2\leq_{A} k_2\cdot d'$ and $d'< d_2$. In such a case, we write $(d_1,d_2)=\interfacePost(b_1)$. When it is clear from the context that $b_2=\interfaceBool(b_1)$, we may write $(d_1,d_2)=\interfacePost(b_1,b_2)$ for readability.

For two partitions $\bkat_1$ and $\bkat_2$ of $\bkat$, we say that $\bkat_1\subseteq\bkat_2$ if for any $b_1\in\bkat_1$, there is $b_2\in\bkat_2$ such that $b_1\leq b_2$. We naturally extend this definition to tuples of partitions of boolean algebras in a pointwise manner. Since $\bkat_1$ and $\bkat_2$ are partitions, it follows that, if $\bkat_1\subseteq \bkat_2$, then for each $b_1\in\bkat_1$ there is exactly one $b_2\in\bkat_2$ with $b_1\leq b_2$. We denote this with the mapping $\bcovers$ from $\bkat_1$ to $\bkat_2$.

Let $\interfaceRel_1$ and $\interfaceRel_2$ be two trace-refinement relations, such that $\proj{1}{\interfacePostS{1}}\subseteq\domain{\interfaceRel_2}$, and let this relationship be captured by the mapping $\bcovers$. We denote with $\interfaceRel_2\circ \interfaceRel_1$ the \emph{composition} of $\interfaceRel_1$ with $\interfaceRel_2$, mapping any element $b_1\in\domain{\interfaceRel_1}$ to the pair $(e_2,A_1\cup A_2)$, where $A_1=\interfaceHypothesesS{1}(b_1)$ and $A_2=\interfaceHypothesesS{2}(e_1)$, where $e_1$ is the element $\bcovers(\proj{1}{\interfacePost(b_1)})$.

\timos{A series of small lemmas that should go to Appendix}

\begin{lemma}\label{lem:superset-hypotheses}
	Suppose that $k_1,k_2\in\kat$ and $A$ a set of hypotheses such that $k_1\leq_{A} k_2$. Then for any $A'$ with $A\subseteq A'$, $k_1\leq_{A'} k_2$.
\end{lemma}

\begin{lemma}\label{lem:kat-less-product}
	Let $k_1,k_2,l_1$ and $l_2$ be elements of a KAT $\kat$. If $k_1\leq l_1$ and $k_2\leq l_2$, then $k_1\cdot k_2\leq l_1\cdot l_2$.
\end{lemma}

\begin{proof}
	We want to show that $k_1\cdot k_2+l_1\cdot l_2 = l_1\cdot l_2$. Notice that $k_1+l_1=l_1$ and $k_2+l_2=l_2$. Therefore, $k_1\cdot k_2+l_1\cdot l_2=k_1\cdot k_2+(k_1+l_1)\cdot (k_2+l_2)=k_1\cdot k_2+k_1\cdot k_2+k_1\cdot l_2+l_1\cdot k_2+l_1\cdot l_2=k_1\cdot k_2+k_1\cdot l_2+l_1\cdot k_2+l_1\cdot l_2=(k_1+l_1)\cdot (k_2+l_2)=l_1\cdot l_2$ as required.
	
\end{proof}

\begin{lemma}\label{lem:kat-less-elements}
	Let $k_1,k_2\in\kat$. It holds that $k_1\leq k_2$ if and only if for all $m\in\kat$, $m\leq k_1$ implies $m\leq k_2$.
\end{lemma}

\begin{proof}
	For the \emph{if} direction, suppose that for all $m\in\kat$, $m\leq k_1$ implies $m\leq k_2$. Then in particular, for $m=k_1$, $k_1\leq k_1$ implies that $k_1\leq k_2$.
	
	For the \emph{only if} direction, suppose that $k_1\leq k_2$, and suppose for contradiction that there is $m\in\kat$ such that $m\leq k_1$ but $m\not\leq k_2$. Then $m+k_1=k_1$, but $m+k_2\neq k_2$. From the assumption that $k_1\leq k_2$, it follows that $k_1+k_2=k_2$. Thus $k_1+m+k_2=k_2$, which implies that $m+k_2=k_2$. It follows that $m\leq k_2$, which is a contradiction.
\end{proof}

\timos{Lemmas for intersection}

\begin{lemma}\label{lem:intersection-distribution-right}
	Let $k,l,o,p$ be elements of some KAT $\kat$, and let $o\leq k$ and $p\leq l$. Then $(k\cdot l)\cap(o\cdot p)\leq (k\cap o)\cdot (l\cap p)$.
\end{lemma}

\begin{proof}
	By definition of intersection, we have that $(k\cdot l)\cap(o\cdot p)\leq o\cdot p$. Since $o\leq k$ and $p\leq l$, by Lemma~\ref{}, we have that $k\cap o=o$ and $l\cap p=p$. Therefore $(k\cdot l)\cap(o\cdot p)\leq (k\cap o)\cdot (l\cap p)$ as required.
\end{proof}

\begin{lemma}\label{lem:intersection-distribution-left}
	Let $k,l,o,p$ be elements of some KAT $\kat$. Then $(k\cap o)\cdot (l\cap p)\leq (k\cdot l)\cap(o\cdot p)$.
\end{lemma}

\begin{proof}
	Let $m$ be any element in $\kat$, such that $m\leq(k\cap o)\cdot (l\cap p)$. Then, by Lemma~\ref{}, there exist $m_1,m_2\in\kat$ such that $m=m_1\cdot m_2$ and $m_1\leq k\cap o$ and $m_2\leq l\cap p$. This means that $m_1\leq k$ and $m_1\leq o$. Similarly, $m_2\leq l$ and $m_2\leq p$. By Lemma~\ref{lem:kat-less-product}, $m_1\cdot m_2\leq k\cdot l$ and $m_1\cdot m_2\leq o\cdot p$. It follows that $m=m_1\cdot m_2\leq (k\cdot l)\cap (o\cdot p)$. Since $m$ was chosen arbitrarily, we have that $(k\cap o)\cdot (l\cap p)\leq (k\cdot l)\cap(o\cdot p)$ by Lemma~\ref{lem:kat-less-elements}.
\end{proof}

\timos{Define the new composition of trace-refinement relations $\interfaceRel_k\circ\interfaceRel_l$.}

\begin{theorem}\label{thm:compositional}
	Suppose $k_1,k_2,l_1$ and $l_2$ are KAT formulas. Let $\interfaceRel_k$ and $\interfaceRel_l$ be trace-refinement relations, such that $\abskrefines{k_1}{k_2}{\interfaceRel_k}$ and $\abskrefines{l_1}{l_2}{\interfaceRel_l}$. Then $\abskrefines{k_1\cdot l_1}{k_2\cdot l_2}{\interfaceRel_k\circ \interfaceRel_l}$.
\end{theorem}

\begin{proof}
	We want to show that for any tuple $(x,y,D)\in\interfaceRel_k\circ\interfaceRel_l$, $(k_1\cdot k_2)\cap x\leq_D(l_1\cdot l_2)\cap y$. Choose such an arbitrary tuple $(x,y,D)\in\interfaceRel_k\circ\interfaceRel_l$, and let $(o,q,A)\in\interfaceRel_k$ and $(p,r,B)\in\interfaceRel_l$ be the tuples that produced $(x,y,D)$. In other words, $x=o\cdot p$, $y=q\cdot r$ and $D=A\cup B$.
	
	Since $\proj{1}{\interfaceRel_k}$ partitions $k_1$ and $\proj{1}{\interfaceRel_l}$ partitions $l_1$, we have that for any $o\in\proj{1}{\interfaceRel_k}$ and $p\in\proj{1}{\interfaceRel_l}$, $o\leq k$ and $p\leq l$, and thus by Lemma~\ref{lem:intersection-distribution-right}, we have that $(k_1\cdot l_1)\cap (o\cdot p)\leq (k_1\cap o)\cdot (l_1\cap p)$.
	% Let $(o,q,A)$ be any tuple in $\interfaceRel_k$ and $(p,r,B)$ be any tuple in $\interfaceRel_l$.
	By assumption, $k_1\cap o\leq_A k_2\cap q$ and $l_1\cap p\leq_B l_2\cap r$. Since $D=A\cup B$, by Lemma~\ref{lem:superset-hypotheses}, we have that $k_1\cap o\leq_{D} k_2\cap q$ and $l_1\cap p\leq_{D} l_2\cap r$. Therefore, by Lemma~\ref{lem:kat-less-product}, we have that $(k_1\cap o)\cdot(l_1\cap p)\leq_D(k_2\cap q)\cdot(l_2\cap r)$. By Lemma~\ref{lem:intersection-distribution-left}, we have that $(k_2\cap q)\cdot(l_2\cap r)\leq_D (k_2\cdot l_2)\cap (q\cdot r)$, and hence $(k_1\cdot l_1)\cap (o\cdot p)\leq_D (k_2\cdot l_2)\cap (q\cdot r)$ as required.
\end{proof}

\timos{old refinement composition below}

\begin{theorem}
	Suppose $k_1,k_2,l_1$ and $l_2$ are KAT formulas. Let $\interfaceRel_k$ and $\interfaceRel_l$ be trace-refinement relations, such that $\abskrefines{k_1}{k_2}{\interfaceRel_k}$ and $\abskrefines{l_1}{l_2}{\interfaceRel_l}$. If $\proj{1}{\interfacePostS{k}}\subseteq\domain{\interfaceRel_l}$, then $\abskrefines{k_1\cdot l_1}{k_2\cdot l_2}{\interfaceRel_l\circ \interfaceRel_k}$.
\end{theorem}

\begin{proof}
	According to Definition~\ref{def:kat-refinement}, we want to show that for all $b_1\in\domain{\interfaceRel_l\circ\interfaceRel_k}$, there exists $b_2\in\bkat$ and set of hypotheses $A\subseteq\hypotheses$, such that $b_1\cdot k_1\cdot l_1\leq_{A}b_2\cdot k_2\cdot l_2$. Notice that
	\begin{displaymath}
		\begin{array}{rl}
			b_1\cdot k_1\cdot l_1 = & b_1\cdot k_1\cdot 1\cdot l_1\\
			= & b_1\cdot k_1\cdot (e_1+\ldots+e_n)\cdot l_1,
		\end{array}
	\end{displaymath}
	where $\{e_1,\ldots,e_n\}$ is the domain of $\interfaceRel_l$ which is a partition by definition of a trace-refinement relation.
	Let $e_i$ be the unique element from $\{e_1,\ldots,e_n\}$ such that $b_1\cdot k_1\leq k_1\cdot e_i$. The existence of such $e_i$ is guaranteed by the assumption that $\proj{1}{\interfacePostS{k}}\subseteq\domain{\interfaceRel_l}$, and its uniqueness is guaranteed by the assumption that $E$ is a partition. Therefore, for all $e_j\neq e_i$, it holds that $b_1\cdot k_1\cdot e_j\leq k_1\cdot e_i\cdot e_j=0$ which implies that $b_1\cdot k_1\cdot e_j=0$. Thus, the above is equal to
	\begin{displaymath}
		\begin{array}{rl}
			b_1\cdot k_1\cdot e_1\cdot l_1+\ldots+b_1\cdot k_1\cdot e_n\cdot l_1 = & b_1\cdot k_1\cdot e_i\cdot l_1.
		\end{array}
	\end{displaymath}
	By the assumption that $\abskrefines{k_1}{k_2}{\interfaceRel_k}$ and $\abskrefines{l_1}{l_2}{\interfaceRel_l}$, there exist $b_2,A_k,e_i'$ and $A_l$, such that
	$b_1\cdot k_1\leq_{A_k} b_2\cdot k_2$ and $e_i\cdot l_1\leq_{A_l}e'_i\cdot l_2$.
	% There is unique $e'$ such that $b_2\cdot k_2\leq k_2\cdot e'$ and $e\cdot l_1\leq_{A_k} e'\cdot l_2$.
	Let $A=A_k\cup A_l$. By Lemma~\ref{lem:superset-hypotheses}, $b_1\cdot k_1\leq_{A} b_2\cdot k_2$ and $e_i\cdot l_1\leq_{A}e'_i\cdot l_2$.
	Then it follows that $b_1\cdot k_1\cdot e_i\cdot l_1\leq_{A} b_2\cdot k_2\cdot e'_i\cdot l_2\leq_{A} b_2\cdot k_2\cdot l_2$, as required.
	
	% We want to show that for any $(b_1,b_2)\in\domain{I_l\circ I_k}=\domain{I_k}$, it holds that $b_1\cdot k_1\cdot l_1\leq_{I_l\circ I_k(b_1,b_2)} b_2\cdot k_2\cdot l_2$. Fix $b_1$ and $b_2$, and let $A=I_l\circ I_k(b_1,b_2)$ and $A_k=I_k(b_1,b_2)$. By assumpion, it holds that $b_1\cdot k_1\leq_{A_k}b_2\cdot k_2$. For $i\in\{1,2\}$, let $d_i$ be an element of $\bkat$, such that $b_i\cdot k_i\leq k_i\cdot d_i$, and there is no $d'\in\bkat$ such that $b_i\cdot k_i\leq k_i\cdot d'$ and $d'\leq d_i$. Thus $(d_1,d_2)=\vec{I_k}(b_1,b_2)$. By assumption, since $\vec{I_k}\subseteq\domain{I_l}$, it follows that there is a tuple $(e_1,e_2)$ in $\domain{I_l}$, such that $d_1\leq e_1$ and $d_2\leq e_2$. Let $A_l=I_l(e_1,e_2)$. By definition $A=A_k\cup A_l$.
%
% 	Firstly, notice that $b_1\cdot k_1\leq_{A_k} b_2\cdot k_2$ and $e_1\cdot l_1\leq_{A_l} e_2\cdot l_2$. From the first relation, we obtain that $k_1\cdot e_1\leq k_2\cdot e_2$. Thus we have the following two equations.
% 	\begin{enumerate}
% 		\item $k_1\cdot e_1+k_2\cdot e_2=k_2\cdot e_2$, and
% 		\item $e_1\cdot l_1+e_2\cdot l_2=e_2\cdot l_2$.
% 	\end{enumerate}
% 	Then
% 	\begin{displaymath}
% 		\begin{array}{rl}
% 			k_2\cdot e_2\cdot l_2 = & k_2\cdot e_2\cdot e_2\cdot l_2\\
% 			= & (k_1\cdot e_1+k_2\cdot e_2)\cdot(e_1\cdot l_1 + e_2\cdot l_2)\\
% 			= & k_1\cdot e_1\cdot e_1\cdot l_1+k_1\cdot e_1\cdot e_2\cdot l_2+k_2\cdot e_2\cdot e_1\cdot l_1+k_2\cdot e_2\cdot e_2\cdot l_2\\
% 			= & k_1\cdot e_1\cdot e_1\cdot l_1+m+k_2\cdot e_2\cdot e_2\cdot l_2\\
% 			= & k_1\cdot e_1\cdot l_1+m+k_2\cdot e_2\cdot l_2\\
% 		\end{array}
% 	\end{displaymath}
% 	Therefore, $k_1\cdot e_1\cdot l_1\leq k_2\cdot e_2\cdot l_2$.
\end{proof}


\timos{Remove or change what follows}

Let $\kat$ be a KAT over the Boolean Algebra $\bkat$. Let $k\in\kat$ and $p,q\in\bkat$. We call the pair $(p,q)$ a \emph{context} of $k$ if $p\cdot k\leq k\cdot q$. Let $p\in\bkat$. We call a set $\{b_1,\ldots,b_n\}$ a \emph{partition} of $p$, if $b_1+b_2+\ldots+b_n\leq b$ and for all $i\neq j\leq n$, $b_i\cdot b_j\equiv 0$.

Given two contexts $c_1=(p_1,q_1)$ and $c_2=(p_2,q_2)$, we define their \emph{composition}, denoted by $c_1\circ c_2$, to be the tuple $(p_1,q_2)$, when $q_1\leq p_2$, and to be undefined otherwise. In the latter case we denote this by writting $c_1\circ c_2 = \bot$.

\begin{lemma}
	Let $k_1,k_2\in\kat$ with respective contexts $c_1=(p_1,q_1)$ and $c_2=(p_2,q_2)$. If $(p_1,q_2)=c_1\circ c_2$, then $(p_1,q_2)$ is a context of $k_1\cdot k_2$.
\end{lemma}

\begin{proof}
	$p_1\cdot k_1\cdot k_2\leq k_1\cdot q_1\cdot k_2\leq k_1\cdot p_2\cdot k_2\leq k_1\cdot k_2\cdot q_2$.
\end{proof}

A \emph{trace context} of a KAT formula $k$ is a tuple $(p,k',q)$ where $k'$ is a KAT formula, and $(p,q)$ is a context of the KAT formula $k\cap k'$. Informally, $k'$ is a KAT formula that restricts the traces described by the input KAT formula $k$.

\subsection{Trace-refinement relations}

\timos{Remove the following, but check before.}

Let $C$ be an arbitrary class of hypotheses for a KAT $k$, and let $r\in C$. We denote with $k|_r$ the KAT obtained by applying the hypothesis $r$ on $k$ and by $k|_C$ by applying all the hypotheses in $C$ on $k$.

Given two KAT formulas $k_1$ and $k_2$, we define an \emph{interface} to be a tuple $(c_1,c_2,r)$ where $c_1$ and $c_2$ are trace contexts of $k_1$ and $k_2$ respectively, and $r$ is a set of hypotheses for the KAT formulas $k_1$ and $k_2$. 

\timos{Discussion on the following.}

{\bf Classes of hypotheses:} For this work, we will explore the effect of just a few types of classes of hypotheses. In general, checking equality of KAT formulas under arbitrary additional hypotheses, can be undecidable \timos{cite/show}. We thus focus on the following types of hypotheses:
\begin{itemize}
	\item Hypotheses that ignore certain actions: $a\equiv 1$, where $a\in\actions$.
	\item Hypotheses that express commutativity of actions or tests against other actions or tests: $a\cdot b\equiv b\cdot a$, where $a,b\in\Sigma$.
\end{itemize}


==> refinement-old.tex <==
%!TEX root = paper.tex
\section{Of Temporal Logic and Refinements}

\timos{I think it's here where we have to define the problem.}

Let $\ap$ be a set of atomic proposition, and assume that the set is the disjoint union of $\ap_B$ and $\ap_E$, corresponding respectively to atomic propositions related to boolean variable checks and assignments, and events.

\timos{$\start{\varphi}$ means that $\varphi$ can only hold in the beginning of the trace. $\last{\varphi}$ means it holds in the end, and only there.}

$$\start{\varphi}\defined \lnext{\globally{\lnot\varphi}}$$

$$\last{\psi}\defined \globally(\lnext{(\false)}\leftrightarrow\psi)$$

For a set of atomic propositions $\ap$, let $\logic{\ap}$ denote the class of logic formulas over $\ap$. For a formula $\varphi\in\logic{\ap}$ and an abstract transition system $\ats$, we denote by $\ats^{\varphi}$, the abstract transition system, such that $\lang{\ats^{\varphi}}=\lang{\ats}\cap\lang{\varphi}$. Additionally, for a subset $A$ of $\ap$, we denote with $\lang{\ats_{|A}^{\varphi}}$ the language $\lang{(\ats'_{|A})}$, where $\ats'=\ats^{\varphi}$. Given an abstract transition system $\ats$, we call a pair of formulas $(\varphi,\psi)\in\logic{\ap}$ a \emph{logical context} of $\ats$, if $\ats\models\start{\varphi}\land(\varphi\rightarrow\last{\psi})$. We denote the set of all logical contexts of some $\ats$ by $\lcontext{\ats}{\ap}$.

A set of formulas $\Phi$ is a partition of $\ats$, if $\bigcup_{\varphi\in\Phi}\lang{\ats^{\varphi}}=\lang{\ats}$ and for any two distinct $\varphi,\psi\in\Phi$ it holds that $\lang{\ats^{\varphi\land\psi}}=\emptyset$. We extend the definition of a partition to work over logical contexts, and we say that a set $C$ of logical contexts is a partition of $\ats$, if the set $\{\phi\mid (\phi,\psi)\in C\}$ is a partition of $\ats$.


 Let $\ats_{1}$ and $\ats_{2}$ be two abstract transition systems over the same set of atomic propositions $\ap$. We aim to find a set $\interface\subseteq \lcontext{\ats_{2}}{\ap_B}\times\lcontext{\ats_{2}}{\ap_B}\times\powset{\ap}$ of \emph{interfaces} for $\ats_{1}$ and $\ats_{2}$, whose elements are tuples of two logical contexts $(\varphi_1,\psi_1)$ and $(\varphi_2,\psi_2)$ of $\ats_{1}$ and $\ats_{2}$ respectively, and a subset $A$ of $\ap$, such that:
\begin{itemize}
	\item the sets $\proj{1}{\interface}$ and $\proj{2}{\interface}$ are partitions of $\ats_{1}$ and $\ats_{2}$ respectively, and
	\item for each $((\varphi_1,\psi_1),(\varphi_2,\psi_2),A)$ in $\interface$, $\lang{(\ats_{1}^{\varphi_1})_{|A}}=\lang{(\ats_{2}^{\varphi_2})_{|A}}$.
\end{itemize}

\timos{Is this compositional? If so, under what assumptions?}

\timos{example}

Let $\ats_{1,1}$, $\ats_{1,2}$, $\ats_{2,1}$, and $\ats_{2,2}$ be abstract transition systems over the same set of atomic propositions $\ap$, with respective contexts $\lcontext{\ats_{1,1}}{\ap_B}$, $\lcontext{\ats_{1,2}}{\ap_B}$, $\lcontext{\ats_{2,1}}{\ap_B}$ and $\lcontext{\ats_{2,2}}{\ap_B}$. Furthermore, let $\interface_1\subseteq \lcontext{\ats_{1,1}}{\ap_B}\times\lcontext{\ats_{2,1}}{\ap_B}\times\powset{\ap}$ and $\interface_2\subseteq \lcontext{\ats_{1,2}}{\ap_B}\times\lcontext{\ats_{2,2}}{\ap_B}\times\powset{\ap}$ be interfaces for $\ats_{1,1}$ and $\ats_{2,1}$, and $\ats_{1,2}$ and $\ats_{2,2}$ repsectively. We define the composition of $\interface_1$ and $\interface_2$ to be the set of tuples $((\chop{(\varphi_1\land\psi)}{ \varphi},\psi_1),(\chop{(\varphi_2\land\psi')}{\varphi'},\psi_2),A)$ such that
there exist tuples $((\varphi_1,\psi),(\varphi,\psi_1),A_1)\in\interface_1$ and $((\varphi_2,\psi'),(\varphi',\psi_2),A_2)\in\interface_2$ where $A= A_1\cup A_2$.
% \begin{itemize}
% 	\item $\psi$ implies $\varphi$,
% 	\item $\psi'$ implies $\varphi'$, and
% 	\item $A= A_1\cup A_2$.
% \end{itemize}
We denote the composition of $\interface_1$ with $\interface_2$ by $\interface_1\circ\interface_2$.

\begin{lemma}\label{lem:projection-subset}
	Let $\ats_1$ and $\ats_2$ be abstract transition systems over $\ap$, and let $A,B\subseteq\ap$, with $A\subseteq B$. Then $\lang{(\ats_{1})_{|B}}=\lang{(\ats_{2})_{|B}}$ implies that $\lang{(\ats_{1})_{|A}}=\lang{(\ats_{2})_{|A}}$.
\end{lemma}

% \begin{lemma}
% 	Let $\ats=\ats_1\circ\ats_2$, and let $(\varphi_1,\psi_1)$ and $(\varphi_2,\psi_2)$ be logical contexts for $\ats_1$ and $\ats_2$ respectively. Then, for any $\path_1\cdot\path_2$ in $\ats$ that satisfies $\chop{\varphi_1}{(\varphi_2\land\psi_1)}$, it holds that $\path_1$
% \end{lemma}

\begin{lemma}
	Let $\ats_{1,1}$, $\ats_{1,2}$, $\ats_{2,1}$, and $\ats_{2,2}$ be abstract transition systems as above with their logical contexts and interfaces, again as defined above. Then $\interface_1\circ\interface_2$ is an interface for $\ats_{1,1}\circ_{\finalstates_{1,1},\initstates_{1,2}}\ats_{1,2}$ and $\ats_{2,1}\circ_{\finalstates_{2,1},\initstates_{2,2}}\ats_{2,2}$.
\end{lemma}

\begin{proof}
	We write $\ats_{1}$ for $\ats_{1,1}\circ_{\finalstates_{1,1},\initstates_{1,2}}\ats_{1,2}$ and $\ats_{2}$ for $\ats_{2,1}\circ_{\finalstates_{2,1},\initstates_{2,2}}\ats_{2,2}$.
	First we need to show that for any tuple $((\chop{(\varphi_1\land\psi)}{\varphi},\psi_1),(\chop{(\varphi_2\land\psi')}{\varphi'},\psi_2),A)$ in $\interface$, $(\varphi_1,\psi_1)$ is a logical context of $\ats_{1}$ and $(\varphi_2,\psi_2)$ a logical context of $\ats_{2}$. Let $((\varphi_1,\psi),(\varphi,\psi_1),A_1)\in\interface_1$ and $((\varphi_2,\psi'),(\varphi',\psi_2),A_2)\in\interface_2$ be the tuples that produced the tuple in $\interface$ at hand.
	Then $\ats_{1,1}\models\start{\varphi_1}\land(\varphi_1\rightarrow\last{\psi})$ and $\ats_{1,2}\models\start{\varphi}\land(\varphi\rightarrow\last{\psi_1})$. Let $\chi = \chop{(\varphi_1\land\psi)}{\varphi}$. We want to show that $\ats_1\models\start{\chi}\land(\chi\rightarrow\last{\psi_1})$. Let $\path$ be any path in $\ats_1$. Since $\ats_1=\ats_{1,1}\circ\ats_{1,2}$, it follows that there are paths $\path_{1,1}$ and $\path_{1,2}$ in $\ats_{1,1}$ and $\ats_{1,2}$ respectively, such that $\path=\path_{1,1}\cdot\path_{1,2}$. Then, by definition, $\ats_{1,1},\path_{1,1}\models\start{\varphi_1}\land(\varphi_1\rightarrow\last{\psi})$ and $\ats_{1,2},\path_{1,2}\models\start{\varphi}\land(\varphi\rightarrow\last{\psi_1})$.
	
	We will first show that if $\ats_1,\path\models\chop{(\varphi_1\land\psi)}{\psi_1}$, then the only subpath witnesses $\path_1,\path_2$ for this formula, are equal to $\path_{1,1}$ and $\path_{1,2}$ respectively. Note that the subpath witnesses are such that $\path_1\models\varphi_1\land\psi$ and $\path_2\models\psi_1$.
	
	Suppose this is not the case. Then either $\path_1$ is a strict prefix of $\path_{1,1}$ or $\path_2$ is a strict suffix of $\path_{1,2}$. For the first case, since $\path_1\models\varphi_1\land\psi$, it follows that 
	
	Firstly, this implies that $\ats_1,\path\models\start{\chi}$. That's because, $\ats_{1,1},\path_{1,1}\models\start{\varphi_1}$. Therefore, $\varphi_1$ can only be satisfied at the beginning of $\path_{1,1}$, and thus $\chi$ as well can only be satisfied at the beginning of $\path$, or at a location $i$ of $\path$ larger than $|\path_{1,1}|$. In the latter case, $\varphi$ would have to be satisfied at a location $i>0$ of $\path_{1,2}$ which is not possible since $\path_{1,2}\models\start{\varphi}$. This means $\chi$ can only be satisfied at the beginning of $\path$.
	
	 Suppose then, that $\ats_1,\path\models\chi$. We want to show that $\ats_1,\path\models\last{\psi_1}$. Since $\ats_1,\path\models\chi$, by definition $\ats_1,\path\models\chop{\varphi_1}{(\varphi\land\psi)}$. Therefore, there exist paths $\path'_1$ and $\path'_2$, such that $\path=\path'_1\cdot\path'_2$ and $\ats_1,\path'_1\models\varphi_1$ and $\ats_1,\path'_2\models\varphi\land\psi$.
	It suffices to show that $\path'_1=\path_{1,1}$ and $\path'_2=\path_{1,2}$. Suppose this is not the case. Then either $\path'_2$ is a strict suffix of $\path_{1,2}$ or $\path'_1$ is a strict prefix of $\path_{1,1}$.
	
	In the first case, it means there is $i>0$, such that $\path_{1,2}^{i}\models\varphi$, which is not possible by the fact that $\path_{1,2}\models\start{\varphi}$, a contradiction.
	In the second case, where $\path'_1$ is a strict prefix of $\path_{1,1}$, it means that $\path_{1,1}\models\lnot\last{\psi}$, a contradiction. This shows that $(\varphi_1,\psi_1)$ is a logical context for $\ats_1$. In the same way, it can be shown that $(\varphi_2,\psi_2)$ is a logical context of $\ats_2$. Therefore, for any tuple in $\interface$ the first and second components are logical contexts of $\ats_1$ and $\ats_2$ respectively.
	
	\vspace{10pt}
	Next, we show that the sets $\proj{1}{\interface}$ and $\proj{2}{\interface}$ are partitions of $\ats_1$ and $\ats_2$ respectively. We look at $\ats_1$ and $\proj{1}{\interface}$ only, as the other case is handled similarly.
	Let $\proj{1}{\interface}=\{(\varphi_1,\psi_1),\ldots,(\varphi_n,\psi_n)\}$. For any $i,j\leq n$, consider $\lang{\ats_1^{\varphi_i\land\varphi_j}}$, and let $\path$ be a path in the latter language, and let $\path_1\in\lang{\ats_{1,1}}$ and $\path_2\in\lang{\ats_{1,2}}$ such that $\path=\path_1\cdot\path_2$. The existence of such subpaths is implied by definition of $\ats_1$. Then $\ats_1,\path\models\varphi_i\land\varphi_j$ and thus $\ats_1,\path\models(\chop{\varphi_{i,1}}{(\varphi_{i,2}\land\varphi_{i,3})})\land(\chop{\varphi_{j,1}}{(\varphi_{j,2}\land\varphi_{j,3})})$, for formulas $\varphi_{i,1},\ldots,\varphi_{j,3}$ obtained from the respective tuples in the interfaces $\interface_1$ and $\interface_{2}$ that generated the tuple in the interface $\interface$.
	Then there are subpaths $\path_{i,1}$ and $\path_{i,2}$, as well as subpaths $\path_{j,1}$ and $\path_{j,2}$, such that
	$$\path_{i,1}\models\varphi_{i,1},\hspace{20pt}\path_{i,2}\models\varphi_{i,2}\land\varphi_{i,3},\hspace{20pt}\path_{j,1}\models\varphi_{j,1},\hspace{20pt}\path_{j,2}\models\varphi_{j,2}\land\varphi_{j,3},$$
	and $\path=\path_{i,1}\cdot\path_{i,2}=\path_{j,1}\cdot\path_{j,2}$.
	First we will show that $\path_{i,1}=\path_{j,1}=\path_1$ and $\path_{i,2}=\path_{j,2}=\path_2$. Consider the case for $i$ first. As before, if $\path_{i,1}\neq\path_1$ and $\path_{i,2}\neq\path_2$, then either $\path_1$ is a strict prefix of $\path_{i,1}$, or $\path_2$ is a strict suffix of $\path_{i,2}$.
	Consider the first case. By definition, either $\path_{i,1}\models\last{\varphi_{i,2}}$ or $\path_{i,1}\models\last{\varphi_{i,3}}$. Let $\psi_i$ be that formula. Then, since $\path_1$ is a strict prefix of $\path_{i,1}$, 
	
	
	\timos{Here we can again show that we can only cut $\path$ at the same point for the two chop formulas.}
	
	\vspace{10pt}
	Finally, we need to show that for any $((\varphi_1,\psi_1),(\varphi_2,\psi_2),A)\in\interface$, $\lang{(\ats_1^{\varphi_1})_{|A}}=\lang{(\ats_2^{\varphi_2})_{|A}}$.
	% Then, $\varphi_1\rightarrow\last{\psi}$ and $\varphi'\rightarrow\last{\psi_1}$. Since by definition $\psi\rightarrow\varphi$, it follows that $\varphi_1\rightarrow\last{\psi_1}$. It can similarly be shown that $\varphi_2\rightarrow\last{\psi_2}$.
\end{proof}
